Understanding the Generalization of In-Context Learning in Transformers: An Empirical Study

Large language models (LLMs) like GPT-4 and LLaMA-3 utilize the powerful in-context learning (ICL) capability of Transformer architecture to learn on the fly from limited examples. While ICL underpins many LLM applications, its full potential remains hindered by a limited understanding of its generalization boundaries and vulnerabilities. We present a systematic investigation of transformers' generalization capability with ICL relative to training data coverage by defining a task-centric framework along three dimensions: inter-problem, intra-problem, and intra-task generalization. Through extensive simulation and real-world experiments, encompassing tasks such as function fitting, API calling, and translation, we find that transformers lack inter-problem generalization with ICL, but excel in intra-task and intra-problem generalization. When the training data includes a greater variety of mixed tasks, it significantly enhances the generalization ability of ICL on unseen tasks and even on known simple tasks. This guides us in designing training data to maximize the diversity of tasks covered and to combine different tasks whenever possible, rather than solely focusing on the target task for testing.

==> paras/func_product_app.tex <==
\section{Additional Experimental Results}
\label{sec:B}
\subsection{Generalization to Products of Learned Functions} \label{4.2}
\label{sec:icl_product}
Moving beyond convex combinations, we explore the generalization of transformers when selecting product combinations (i.e., $\calT_\times$) as the operation on base function classes. Unlike convex combinations, where the model typically aligns with one constituent function to maintain control over squared error (SE), product multiplication allows more freedom in fitting individual function classes, potentially leading to greater divergence from the true product curve. We also consider the combinations of $\calF^{(0)}_1=\{\phi \sin(x): \phi \in \bbR\}$ and $\calF^{(0)}_3=\{\phi \sin(2x): \phi \in \bbR\}$ as the extra function classes to train the ComFuncLearner model here.

\begin{table*}[t]
    \centering
    \small
    \caption{SE of the ComFuncLearner and Baseline model tested on the products of base functions. CFL1, CFL2, and CFL4 indicate CFL with 1, 2, and 4 combinations of base functions in its training data, respectively.}
  
    \resizebox{\linewidth}{!}{
    \vspace{-0px}
    \begin{tabular}{c|c|ccccc|cccccccc}
        \toprule

         Range & Model & s(x) & c(x) & s(2x) & c(2x) & Mean$\rm{_B}$ & s(x)\&c(x) & s(x)\&s(2x) & s(x)\&c(2x) & c(x)\&s(2x) & c(x)\&c(2x) & s(2x)\&c(2x) & Com$\_$All & Mean$\rm{_C}$
                   \\
        \midrule
        \multirow{4}{*}{1-10}  & Baseline & 3.50e-3          & 3.65e-3          & 5.34e-3          & 5.29e-3          & 4.45e-3          & 2.87e-2          & 1.89e-2          & 7.19e-2          & 2.10e-2          & 2.85e-2          & 1.44e-2          & 4.14e-2          & 3.21e-2          \\
                       & CFL1     & 4.04e-3          & 2.71e-3          & 4.01e-3          & 4.87e-3          & 3.91e-3          & 2.83e-2          & \textbf{5.90e-3} & 4.28e-2          & 1.45e-2          & 2.65e-2          & 1.98e-2          & 3.59e-2          & 2.48e-2          \\
                       & CFL2     & 4.85e-3          & 3.46e-3          & \textbf{2.35e-3} & \textbf{3.23e-3} & \textbf{3.47e-3} & \textbf{4.96e-3} & 2.31e-2          & 3.52e-2          & 1.37e-2          & 2.42e-2          & \textbf{4.85e-3} & \textbf{2.27e-2} & 1.84e-2          \\
                       & CFL4     & \textbf{3.42e-3} & \textbf{2.63e-3} & 4.13e-3          & 4.19e-3          & 3.59e-3          & 5.95e-3          & 5.94e-3          & \textbf{2.61e-2} & \textbf{1.35e-2} & \textbf{6.01e-3} & 7.16e-3          & 2.70e-2          & \textbf{1.31e-2} \\ 
        \midrule
        \multirow{4}{*}{11-20} & Baseline & 4.54e-5          & 1.17e-5          & 2.13e-5          & 6.46e-5          & 3.61e-5          & 2.81e-2          & 9.07e-3          & 5.21e-2          & 1.35e-2          & 1.69e-2          & 7.65e-3          & 4.87e-2          & 2.52e-2          \\
                               & CFL1     & \textbf{2.77e-5} & 9.16e-6          & 4.04e-5          & \textbf{5.06e-5} & \textbf{3.23e-5} & 8.57e-3          & \textbf{9.40e-5} & 1.78e-2          & 5.78e-3          & 1.96e-2          & 3.23e-3          & 2.16e-2          & 1.10e-2          \\
                               & CFL2     & 3.53e-5          & \textbf{5.23e-6} & \textbf{1.93e-5} & 8.22e-5          & 3.61e-5          & \textbf{4.49e-5} & 1.22e-2          & \textbf{1.15e-2} & 8.44e-3          & 1.59e-2          & \textbf{1.30e-4} & \textbf{1.36e-2} & 8.85e-3          \\
                               & CFL4     & 4.08e-5          & 1.18e-5          & 4.34e-5          & 6.92e-5          & 4.12e-5          & 5.09e-5          & 1.88e-4          & 6.92e-3          & \textbf{5.27e-3} & \textbf{1.07e-3} & 2.55e-4          & 1.59e-2          & \textbf{4.11e-3} \\
        \midrule
        \multirow{4}{*}{21-30} & Baseline & 3.28e-5          & 7.39e-6          & 1.58e-5          & 4.18e-5          & 2.43e-5          & 2.67e-2          & 7.69e-3          & 3.29e-2          & 8.85e-3          & 1.56e-2          & 5.70e-3          & 5.16e-2          & 2.13e-2          \\
                               & CFL1     & \textbf{1.94e-5} & 6.75e-6          & 3.23e-5          & 3.42e-5          & 2.38e-5          & 4.45e-3          & \textbf{5.41e-5} & 9.81e-3          & \textbf{3.05e-3} & 1.45e-2          & 1.68e-3          & 1.42e-2          & 6.83e-3          \\
                               & CFL2     & 2.48e-5          & \textbf{3.28e-6} & \textbf{1.17e-5} & 6.98e-5          & 2.73e-5          & 3.47e-5          & 1.03e-2          & 8.66e-3          & 6.21e-3          & 1.35e-2          & \textbf{9.78e-5} & \textbf{1.06e-2} & 7.05e-3          \\
                               & CFL4     & 2.33e-5          & 6.69e-6          & 1.56e-5          & \textbf{3.36e-5} & \textbf{2.03e-5} & \textbf{2.76e-5} & 1.16e-4          & \textbf{2.99e-3} & 3.39e-3          & \textbf{4.23e-5} & 1.08e-4          & 1.38e-2          & \textbf{2.94e-3} \\
        \midrule
        \multirow{4}{*}{31-40} & Baseline & 2.52e-5          & 7.24e-6          & 1.61e-5          & 3.71e-5          & 2.17e-5          & 2.69e-2          & 7.76e-3          & 2.48e-2          & 8.86e-3          & 8.52e-3          & 5.21e-3          & 5.06e-2          & 1.98e-2          \\
                               & CFL1     & 1.82e-5          & 6.75e-6          & 3.65e-5          & 3.07e-5          & 2.31e-5          & 3.16e-3          & \textbf{4.99e-5} & 7.58e-3          & 2.84e-2          & 1.16e-2          & 1.59e-3          & 9.88e-3          & 5.24e-3          \\
                               & CFL2     & 2.44e-5          & \textbf{3.26e-6} & \textbf{1.13e-5} & 6.31e-5          & 2.61e-5          & 2.71e-5          & 8.78e-3          & 6.57e-3          & 5.52e-3          & 1.33e-2          & \textbf{7.83e-5} & 9.02e-3          & 6.21e-3          \\
                               & CFL4     & \textbf{1.79e-5} & 5.44e-6          & 1.25e-5          & \textbf{2.49e-5} & \textbf{1.57e-5} & \textbf{2.02e-5} & 9.73e-5          & \textbf{2.23e-3} & \textbf{2.77e-3} & \textbf{3.40e-5} & 8.77e-5          & \textbf{7.01e-3} & \textbf{2.24e-3} \\ 
        \bottomrule
    \end{tabular}
    }
    \label{tab:se_product}
\end{table*}


\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/mul_v2.pdf}
    \caption{Function curves on the product combinations of base functions fitted by models after ICL. The product combination used via training phase is $\calF_1\text{ and }\calF_2$.}
    \label{fig:se_product_0}
\end{figure*}

Table \ref{tab:se_product} reveals the Baseline model's persistent struggle to accurately predict product combinations within the ICL. Despite having witnessed only one combinatorial pattern, the ComFuncLearner model consistently surpasses the Baseline in this task. However, compared to the substantial improvement observed in convex combination experiments, the ComFuncLearner's advantage in product combinations is less pronounced. We hypothesize that this disparity arises from the inherent difficulty of fitting product combinations compared to convex combinations. 

To investigate this further, we progressively increase the number of product combinations presented to the ComFuncLearner model in subsequent experiments (1, 2, 3, and 4). Specifically, we report the results of the ComFuncLearner model combinational function classes including \{$\calF^{(0)}_1 \times \calF^{(0)}_3$, $\calF^{(0)}_1 \times \calF^{(0)}_2$, $\calF^{(0)}_2 \times \calF^{(0)}_4$, $\calF^{(0)}_3 \times \calF^{(0)}_4$\}. 
Please note that we only add more patterns of combinations to the training yet the number of all training samples and training steps are fixed the same for the Baseline model, the ComFuncLearner model with 1, 2, and 4 combinations in its training.


This manipulation aims to determine whether exposure to a wider range of combinatorial patterns during training could enhance the model's generalization ability to unseen product combinations. As shown in Table \ref{tab:se_product}, we observe a consistent decrease of SE as the number of product combination patterns presented to the ComFuncLearner model in the training increases. For example, we observe the mean SE among 21-31 points drop from 0.0231 (the Baseline model) to 0.00294 (the ComFuncLearner with 4 combination patterns in its training data). Figure \ref{fig:se_product_0} presents the function curves learned after 39 examples and reveals a distinct trend: as the number of seen combinations in training increases, the model's fit to the objective function steadily improves. With 4 combinations observed, the ComFuncLearner model's fit closely approximates the true function's curve.
This suggests that when we select product combination as the operation on base functions, transformers fail to achieve inter-problem generalization but show intra-problem generalization, which can be improved as the number of learned combinations increases. 






==> paras/limitations.tex <==
\section{Limitations and Broader Impacts} \label{sect:limiation}
While our study provides valuable insights into the generalization capabilities of Large Language Models (LLMs) like GPT-3 with in-context learning (ICL), several limitations exist. Our investigation primarily focuses on a task-centric framework that may not encompass all real-world scenarios and variations. The observed vulnerability of ICL to distribution shifts highlights the need for further research to enhance robustness and reliability.

The broader impacts of our findings emphasize the necessity for ongoing development of more adaptable and resilient LLMs, particularly for applications in dynamic and sensitive fields where performance reliability is critical. This research underscores the importance of advancing our understanding of LLM generalization to foster their safe and effective deployment in diverse real-world contexts.


==> paras/other.tex <==

\begin{table*}[t]
    \centering
    \small
    \caption{SE of the 2D ComFuncLearner and Baseline model tested on the convex combinations of base functions. Range indicates the range in each sequence to calculate SE. $\rm{s(\cdot)}$ and $\rm{c(\cdot)}$ represent $\rm{\sin(\cdot)}$ and $\rm{\cos(\cdot)}$, respectively. Mean$\rm{_B}$ and Mean$\rm{_C}$ indicate the mean SE of base functions and combinations of base functions, respectively. Com$\_$All indicates the combination of all base functions.}
    \resizebox{\linewidth}{!}{ 
    \vspace{-0px}
    \begin{tabular}{c|c|ccccc|cccccccc}
    % \begin{tabular}{c|cccccccccccc}
        \toprule
        % {CC+s1s2, baseline+s3}
         Range & Model & s(x) & c(x) & s(2x) & c(2x) & Mean$\rm{_B}$ & s(x)\&c(x) & s(x)\&s(2x) & s(x)\&c(2x) & c(x)\&s(2x) & c(x)\&c(2x) & s(2x)\&c(2x) & Com$\_$All & Mean$\rm{_C}$ \\
        \midrule
        \multirow{2}{*}{1-10} 
        & $\Delta_2$ & 4.30e-3 & 3.84e-3 & 3.36e-3 & 6.90e-4 & 3.05e-3 & 7.64e-3 & 3.85e-3 & 5.23e-3 & 5.03e-3 & 4.42e-3 & 5.63e-3 & 5.37e-3 & 5.30e-3 \\
        & $\Delta_4$ & 1.89e-2 & 1.06e-2 & 1.68e-2 & 8.43e-3 & 1.37e-2 & 1.81e-2 & 2.05e-2 & 1.81e-2 & 1.63e-2 & 9.97e-3 & 1.72e-2 & 2.93e-2 & 1.85e-2 \\
        & $\Delta_8$ & 9.49e-3 & 8.42e-3 & 7.45e-3 & 1.03e-2 & 8.92e-3 & 1.31e-2 & 1.40e-2 &1.51e-2 & 1.29e-2 & 1.36e-2 & 1.49e-2 & 1.97e-2 & 1.48e-2 \\
        \midrule
        \multirow{2}{*}{11-20} 
        & $\Delta_2$ & 5.91e-3 & 1.38e-2 & 2.79e-3 & -4.32e-5 & 5.63e-3 & 8.41e-3 & 2.91e-3 & 4.90e-3 & 5.17e-3 & 7.68e-3 & 5.01e-3 & 3.83e-3 & 5.42e-3 \\
        & $\Delta_4$ & 2.57e-2 & 1.81e-2 & 2.20e-2& 1.67e-2 & 2.06e-2 & 3.11e-2 & 3.68e-2 & 2.83e-2 & 2.73e-2 & 2.16e-2 & 2.45e-2 & 4.75e-2 & 3.10e-2 \\
        & $\Delta_8$ & 1.38e-2 & 1.47e-2 & 1.36e-2 & 1.15e-2 & 1.34e-2 & 2.61e-2 & 2.95e-2 &2.13e-2 & 2.79e-2 & 2.74e-2 & 2.46e-2 & 3.10e-2 & 2.69e-2 \\
        \midrule
        \multirow{2}{*}{21-30} 
        & $\Delta_2$ & 6.58e-3 & 1.42e-2 & 4.39e-3 & -5.35e-4 & 6.15e-3 & 7.35e-3 & 1.54e-3 & 3.52e-3 & 5.18e-3 & 7.95e-3 & 3.95e-3 & 3.82e-3 & 4.76e-3 \\
        & $\Delta_4$ & 2.39e-2 & 1.84e-2 & 2.23e-2 & 1.90e-2 & 2.09e-2 & 3.47e-2 & 3.92e-2 & 3.19e-2 & 3.33e-2 & 2.69e-2 & 3.12e-2 & 5.18e-2 & 3.56e-2 \\
        & $\Delta_8$ & 1.42e-2 & 1.29e-2 & 1.45e-2 & 1.40e-2 & 1.39e-2 & 2.95e-2 & 3.48e-2 &2.97e-2 & 3.23e-2 & 2.68e-2 & 2.79e-2 & 3.68e-2 & 3.11e-2 \\
        \midrule
        \multirow{2}{*}{31-40} 
        & $\Delta_2$ & 6.76e-3 & 2.12e-2 & 4.54e-3 & -2.44e-4 & 8.06e-3 & 7.01e-3 & 2.07e-3 & 3.69e-3 & 6.50e-3 & 8.85e-3 & 3.93e-3 & 4.35e-3 & 5.21e-3 \\
        & $\Delta_4$ & 2.73e-2 & 2.24e-2 & 3.08e-2 & 2.14e-2 & 2.55e-2 & 3.93e-2 & 4.40e-2 & 3.60e-2 & 3.32e-2 & 2.57e-2 & 3.95e-2 & 6.11e-2 & 3.98e-2 \\
        & $\Delta_8$ & 1.36e-2 & 1.50e-2 & 1.66e-2 & 1.13e-2 & 1.41e-2 & 3.56e-2 & 3.34e-2 & 2.81e-2 & 3.36e-2 & 2.89e-2 & 3.07e-2 & 4.31e-2 & 3.34e-2 \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:se_convex}
\end{table*}


\begin{table*}[t]
    \centering
    \small
    \caption{SE of the 2D ComFuncLearner and Baseline model tested on the convex combinations of base functions. Range indicates the range in each sequence to calculate SE. $\rm{s(\cdot)}$ and $\rm{c(\cdot)}$ represent $\rm{\sin(\cdot)}$ and $\rm{\cos(\cdot)}$, respectively. Mean$\rm{_B}$ and Mean$\rm{_C}$ indicate the mean SE of base functions and combinations of base functions, respectively. Com$\_$All indicates the combination of all base functions.}
    \resizebox{\linewidth}{!}{ 
    \vspace{-0px}
    \begin{tabular}{c|c|ccccc|cccccccc}
    % \begin{tabular}{c|cccccccccccc}
        \toprule
        % {CC+s1s2, baseline+s3}
         Range & Model & s(x) & c(x) & s(2x) & c(2x) & Mean$\rm{_B}$ & s(x)\&c(x) & s(x)\&s(2x) & s(x)\&c(2x) & c(x)\&s(2x) & c(x)\&c(2x) & s(2x)\&c(2x) & Com$\_$All & Mean$\rm{_C}$ \\
        \midrule
        \multirow{2}{*}{1-10} 
        & $\Delta_2$ & -3.87e-3 & 2.48e-3 & 4.63e-3 & -2.75e-3 & 1.22e-4 & 4.35e-3 & 4.06e-3 & 7.13e-3 & 6.03e-3 & 1.70e-3 & 7.29e-3 & 5.05e-3 & 5.09e-3 \\
        & $\Delta_4$ & 5.95e-3 & 1.07e-2 & 4.49e-3 & 3.43e-3 & 6.16e-3 & 3.12e-3 & -5.75e-4 & 6.58e-3 & 1.39e-2 & 2.55e-3 & 1.12e-2 & 2.23e-3 & 5.57e-3 \\
        & $\Delta_8$ & 1.62e-3 & 1.35e-2 & 7.62e-3 & 1.36e-2 & 9.08e-3 & 1.16e-2 & 8.96e-3 & 1.43e-2 & 1.87e-2 & 1.63e-2 & 1.00e-2 & 2.62e-2 & 1.52e-2 \\
        \midrule
        \multirow{2}{*}{11-20} 
        & $\Delta_2$ & -4.11e-2 & 2.21e-3 & 3.62e-3 & -9.96e-3 & -2.05e-3 & 6.14e-3 & 9.76e-3 & 1.39e-2 & 5.24e-3 & -2.03e-3 & 9.11e-3 & 3.79e-3 & 6.57e-3 \\
        & $\Delta_4$ & 5.17e-3 & 2.26e-2 & 7.03e-3 & 8.67e-3 & 1.08e-2 & 1.18e-2 & 9.46e-3 & 1.66e-2 & 2.32e-2 & 1.06e-2 & 2.34e-2 & 1.99e-2 & 1.64e-2 \\
        & $\Delta_8$ & 1.25e-2 & 2.48e-2 & 1.52e-2 & 2.09e-2 & 9.08e-3 & 1.16e-2 & 8.96e-3 & 1.43e-2 & 1.87e-2 & 1.63e-2 & 1.01e-2 & 2.62e-2 & 1.52e-2 \\
        \midrule
        \multirow{2}{*}{21-30} 
        & $\Delta_2$ & -2.24e-3 & 3.16e-3 & 4.94e-3 & -1.01e-2 & -1.04e-3 & 6.11e-3 & 1.16e-2 & 1.67e-2 & 5.84e-3 & -3.41e-3 & 9.81e-3 & 5.44e-3 & 7.45e-3 \\
        & $\Delta_4$ & 5.71e-3 & 2.39e-2 & 1.28e-2 & 1.09e-2 & 1.33e-2 & 1.48e-2 & 9.08e-3 & 1.46e-2 & 3.32e-2 & 1.11e-2 & 2.79e-2 & 3.24e-2 & 2.04e-2 \\
        & $\Delta_8$ & 1.14e-2 & 2.81e-2 & 1.93e-2 & 2.26e-2 & 2.04e-2 & 3.81e-2 & 3.26e-2 & 2.49e-2 & 4.06e-2 & 3.86e-2 & 2.75e-2 & 6.23e-2 & 3.78e-2 \\
        \midrule
        \multirow{2}{*}{31-40} 
        & $\Delta_2$ & 4.86e-4 & 3.47e-3 & 6.32e-3 & -9.71e-3 & 1.41e-4 & 7.52e-3 & 1.36e-2 & 1.54e-2 & 6.17e-3 & -3.15e-3 & 1.08e-2 & 6.18e-3 & 8.08e-3 \\
        & $\Delta_4$ & 8.45e-3 & 2.54e-2 & 1.09e-2 & 1.09e-2 & 1.33e-2 & 1.20e-2 & 1.44e-2 & 1.69e-2 & 2.81e-2 & 1.53e-2 & 3.18e-2 & 3.04e-2 & 2.04e-2 \\
        & $\Delta_8$ & 1.23e-2 & 3.10e-2 & 2.05e-2 & 2.73e-2 & 2.28e-2 & 3.71e-2 & 3.96e-2 & 2.73e-2 & 5.35e-2 & 4.04e-2 & 3.46e-2 & 6.48e-2 & 4.24e-2 \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:se_convex}
\end{table*}
